mrCAD: Multimodal Refinement of Computer-aided Designs

A key feature of human collaboration is the ability to iteratively refine the concepts we have communicated. In contrast, while generative AI excels at the \textit{generation} of content, it often struggles to make specific language-guided \textit{modifications} of its prior outputs. To bridge the gap between how humans and machines perform edits, we present mrCAD, a dataset of multimodal instructions in a communication game. In each game, players created computer aided designs (CADs) and refined them over several rounds to match specific target designs. Only one player, the Designer, could see the target, and they must instruct the other player, the Maker, using text, drawing, or a combination of modalities. mrCAD consists of 6,082 communication games, 15,163 instruction-execution rounds, played between 1,092 pairs of human players. We analyze the dataset and find that generation and refinement instructions differ in their composition of drawing and text. Using the mrCAD task as a benchmark, we find that state-of-the-art VLMs are better at following generation instructions than refinement instructions. These results lay a foundation for analyzing and modeling a multimodal language of refinement that is not represented in previous datasets.

==> sections/evaluation__1_.tex <==
\section{Evaluation}
\label{sec:evaluation}
% \begin{table*}[]
%     \centering
%     \small
%     \begin{tabular}{lrrrrrrrrrr}
%     \toprule
%     &  & \multicolumn{9}{c}{\textbf{Vision-language models}} \\
%     \cmidrule(lr){3-11}
%     & \textbf{Human} & \textbf{GPT-4o} & $-\text{drawing}$ & $-\text{text}$ & \textbf{Claude} & \textbf{GPT-4o-mini} & \textbf{Qwen} & \textbf{Qwen FT} & & \\
%     \midrule
%     generation & 0.85 & 0.55 & & & 0.50 & 0.31 & 0.12 & 0.43 & & \\
%     refinement & 0.12 & -0.12 & & & -0.05 & -0.13 & -0.05 & -0.02 & & \\
%     \bottomrule
%     \end{tabular}
%     \caption{Proportional improvement results for vision-language chat models. Claude results are from Claude-3.7-Sonnet, and Qwen results are from Qwen2.5-VL-7B-Instruct. Qwen-7B FT is a Qwen2.5-VL-7B-Instruct model fine-tuned on mrCAD data.}
%     \label{tab:api_results}
% \end{table*}

We evaluate both API access models and open-weights models (which we finetune) on the \mrcad{} dataset. 
We are interested in the following.
\begin{enumerate}[label=\textbf{RQ\arabic*},labelindent=0pt,leftmargin=*,itemsep=0pt,parsep=0pt]
    \item What is the difference in performance between people and models in following the instructions?
    \item What is the effect of generation vs refinement in model performance ?
    \item What is the effect of multi-modal vs single-modal in model performance?
\end{enumerate}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\textwidth]{figs/evals.pdf} % Placeholder image
  \caption{\textbf{A} Comparison of human and model movement towards target following instructions, normalized by distance at start of round. Only humans make reliably positive changes in responses to refinement instructions. Models made positive steps in generation but largely destructive changes when refining. \textbf{B} Comparison of human and model responses.}
  \label{fig:evals}
\end{figure*}

\subsection{Benchmark}
We select CADs from the \textbf{dense set} that have 3 or more successful ($\Delta(D_n, D^*) < 0.2$) rollouts.
This results in $682$ unique CADs with $2324$ rollouts, and a total of $5751$ rounds of instruction-execution pairs.
Then, for these selected rounds, we can evaluate VLM agents by having them assume the role of a human maker $P_\text{maker}$.

\paragraph{Metric}
We evaluate the instruction-following abilities by proportional improvements \textbf{PI}: how much the distance to target $D^*$ shrinks as a consequence of an agent's actions.
\begin{align*}
    \text{PI}(A, R_{:i}, D^*) &= \frac{\Delta(D_i, D^*) - \Delta(A(D_i), D^*)}{\Delta(D_i, D^*)}
\end{align*}
This metric is proportional w.r.t. the amount of remaining distance to target at every round.
This accounts for the fact that distances to the target decrease significantly as rounds progress, making late-stage refinements less noticeable without this normalization.

\subsection{Evaluating vision-language models}

We build a gym framework for standardized evaluations across models. The gym framework allows for instantiating agents that interface with a standardized representation of CADs, and allows for handing the mrCAD dataset, evaluating models, and simulating interactions between designer and maker agents.

We use the gym framework to evaluate multiple vision-language chat models -- both API access and open weights models -- on the mrCAD benchmark, by having these models assume the role of a human maker.
% \begin{small}
    \begin{align*}
        P_\text{model-maker}(A ~|~ m, D_i, R_{1:i-1})
    \end{align*}
% \end{small}

\paragraph{API access models} 
Since we present the rendered interaction history and drawing instructions to the model, we require models that are accept interleaved image-text inputs. We choose the following models off-the-shelf based on this criterion: GPT-4o \cite{openai2024gpt4ocard}, GPT-4o-mini \cite{openai2025gpt4omini}, Claude-3.7-Sonnet \cite{anthropic2025claude37}, and Qwen2.5-VL-7B-Instruct \cite{bai2025qwen25vltechnicalreport}.
To generate editing actions, we prompt the models to generate editing actions as tool calls. 

\paragraph{Finetuned Model}
We also fine-tune a Qwen2.5-VL-7B-Instruct model in the same setting to generate editing actions. We use the 2684 rollouts from the coverage set as a training set. We also include rollouts that don't pass the evaluation threshold. We create a small held-out validation set by choosing 303 successful rollouts from the dense set for 187 CADs that have fewer than 3 successful rollouts for model selection. We train LoRA \cite{hu2022lora} adapters for both vision and language modules of the network.

\begin{table}[]
    \centering
    \begin{tabular}{lrr}
        \toprule
         & \textbf{generation} & \textbf{refinement} \\
        \midrule
        Human & 0.85 & 0.12 \\
        \midrule
        GPT-4o & 0.55 & -0.12 \\
        $-\text{drawing}$ & 0.51 & -0.16 \\
        $-\text{text}$ & 0.54 & -0.12 \\
        \midrule
        Qwen-7B FT & 0.43 & -0.02 \\
        $-\text{drawing}$ & 0.36 & -0.03 \\
        $-\text{text}$ & 0.41 & -0.04 \\
        \midrule
        GPT-4o-mini & 0.31 & -0.13 \\
        Claude-3.7 & 0.50 & -0.05 \\
        Qwen-7B & 0.12  & -0.05 \\
        \bottomrule
        \end{tabular}
        \caption{Proportional improvement results for vision-language chat models, including results on ablated instructions. Claude results are from Claude-3.7-Sonnet, and Qwen results are from Qwen2.5-VL-7B-Instruct. Qwen-7B FT is a Qwen2.5-VL-7B-Instruct model fine-tuned on mrCAD data. 
        % For GPT-4o, we only evaluate with the ablated instructions from the evaluation set, while for Qwen-7B FT we fine-tune the model on the training set with the corresponding modality ablated.
        All models perform worse than humans in following instructions, especially instructions of refinements, where the models' outputs actually make the design worser.
        }
    \label{tab:ft_results}
\end{table}

\paragraph{Ablation on modality}
We ablate one modality (if present) from all the instructions and evaluate them to create $-\text{drawing}$ and $-\text{text}$ evaluation sets. We also perform these ablations on the training data and fine-tune separate Qwen2.5-VL-7B-Instruct models to obtain $\text{Qwen-7B FT}_{-\text{drawing}}$ and $\text{Qwen-7B FT}_{-\text{text}}$ models to 
evaluate on the $-\text{drawing}$ and $-\text{text}$ evaluation sets respectively. We use the same LoRA fine-tuning setup for these experiments.

\subsection{Performance of vision-language models}
For the results, we group rounds as either generation (round 1) and refinement (round 2+). 
Note that this grouping is imprecise and can be improved in future works, as participants do instruct each other to generate in later rounds.

\textbf{RQ1, RQ2} We found (Table~\ref{tab:ft_results}) that models are generally able to decrease the distance to the target during \textit{generation}, with more capable models (GPT-4o, Claude-3.7-Sonnet) and fine-tuned models doing better. However, we find that models perform quite poorly in \textit{refinement} turns. We see that models often make changes that actually \emph{increase} the distance to the target -- in opposition to the intention of the designer's instruction. 
We also see that while an approach like supervised fine-tuning leads to significant improvements in generation turns, the gains don't transfer to refinement turns. This suggests that more sophisticated training approaches might be needed to tackle refinement.

\textbf{RQ3} We also see that models are sensitive to both instruction modalities (Table~\ref{tab:ft_results}), with performance descreasing when a multimodal instruction is ablated to have only a single modality. This effect is more pronounced in generation rounds.

% We found that models were able to decrease distance to the target in generation rounds (Fig.~\ref{fig:evals}A).
% Furthermore, these changes seemed somewhat sensible (Fig.~\ref{fig:evals}B), \textbf{explain the good things it did}.
% However, models were not able follow refinement instructions in a way that decreased distance to the target.
% \textbf{explain any good refinements it did do, and why it appears to be failing}.

% We should really have a baseline to make claims that generation rounds are better than nothing
% It's impossible to make negative changes in round 1

% In discussion: it should not be surprising that models cannot do this, given that data of this type is lacking. \ref{tab:ft_results}





==> sections/related__1_.tex <==
\section{Related Work}

\paragraph{Multimodality}
The instructions in \mrcad{} are multi-modal, consisting of both texts and drawings. 
This is in contrast to other works such as \citet{pejsa2016room2room} and \citet{ku-etal-2020-room}, where the context of the agent is multi-modal, yet the instructions themselves only contain language.
% Our dataset contains many examples of drawings and text that mutually support each other. 
Our drawings efficiently convey spatial information and reference, and even short utterances -- ``delete this'', ``move to here'' -- can hugely constrain the meaning of drawings.
Our work highlights the capacity of drawing to act, not only as a depictive medium, but as a versatile tool for \textit{communication} \cite{goodman1976languages, huey2021semantic, fan2023drawing}, and provides a resource for studying this phenomenon in a grounded way \cite{lachmy2022draw}.

\paragraph{Generating Designs} 
Prior work has explored AI agents that assist with computer aided design tasks, including those that leverage various kinds of input modality \cite{sanghi2022clip, chen2024generic}, including drawings \cite{seff2021vitruvion}. 
Beyond CAD, other work has explored how agents can support various kinds of designs given multimodal inputs, including generating HTML and CSS code \cite{si2024design2code} and slide-shows \cite{ge2025autopresent}. 

\paragraph{Refinement}
The interactions between people in \mrcad{} takes multiple turns, as a dyad collaboratively refine a current CAD toward a specific target. 
% This is in contrast to multimodal instruction-following datasets such as \citet{ku-etal-2020-room} containing a single turn of instruction and response. 
\citet{lachmy2022draw} study complex instructions, but these are presented all at once by the speaker and verified with interpretation by another agent. \mrcad{} prioritizes refinement, where people must elaborate on and repair previous instructions, in this regard, our work is similar to \citet{kim-etal-2019-codraw}.


% \citet{si2024design2code} introduce a front-end design benchmark where an agent is tasked with generating HTML and CSS code, given a visual representation of intent -- the screenshot of the desired page. 
% \citet{ge2025autopresent} develop agents that create a slide given a natural language description of the slide. 
% Our work introduces the task of \emph{refining} designs given \emph{multimodal} instructions in the form of drawings and text.
% \cite{zitnick2013bringing} presents a dataset of comic-book like scene, along with a natural language description of parts are parts, cad parts are fluid.



==> style_dump.tex <==
\iftaclpubformat
\section{Courtesy warning: Common violations of \taclpaper rules that have
resulted in papers being returned to authors for corrections}
fdafsa
Avoid publication delays by avoiding these.



\begin{enumerate}
\item Violation: incorrect parentheses for in-text citations.  See \S
\ref{sec:in-text-cite} and Table \ref{tab:cite-commands}.
\item Violation: URLs that, when clicked, yield an error such as a 404 or go
to the wrong page.
  \begin{itemize}
     \item Advice: best scholarly practice for referencing URLS would be to also
     include the date last accessed.
  \end{itemize}
\item Violation: non-fulfillment of promise from submission to provide access
instructions (such as a URL) for code or data.
\item Violation: References incorrectly formatted (see \S\ref{sec:references}).
Specifically:
\begin{enumerate}
  \item Violation: initials instead of full first/given names in references.
  \item Violation: missing periods after middle initials.
  \item Violation: incorrect capitalization.  For example, change ``lstm'' to
  LSTM and ``glove'' to GloVe.
  \begin{itemize}
    \item Advice: if using BibTex, apply curly braces within the title field to
    preserve intended capitalization.
  \end{itemize}
  \item Violation: using ``et al.'' in a reference instead of listing all
  authors of a work.
  \begin{itemize}
    \item Advice: List all authors and check accents on author names even when
    dozens of authors are involved.
  \end{itemize}
  \item Violation: not giving a complete arXiv citation number.
  \begin{itemize}
     \item Advice: best scholarly practice would be to give not only the full
     arXiv number, but also the version number, even if one is citing version 1.
  \end{itemize}
  \item Violation: not citing an existing peer-reviewed version in addition to
  or instead of a preprints
    \begin{itemize}
     \item Advice: When preparing the camera-ready, perform an additional check
     of preprints cited to see whether a peer-reviewed version has appeared
     in the meantime.
  \end{itemize}
  \item Violation: book titles do not have the first initial of all main words
  capitalized.
  \item Violation: In a title, not capitalizing the first letter of the first word
  after a colon or similar punctuation mark.
\end{enumerate}
\item Violation: figures or tables appear on the first page.
  \item Violation: the author block under the title is not
    formatted according to Appendix~\ref{sec:authorformatting}.
\end{enumerate}
\else
% Submission-specific rules
\section{Courtesy warning: Common violations of \taclpaper rules that have
resulted in desk
rejects}
\begin{enumerate}
  \item Violation: wrong paper format.
  \emph{As of the September 2018 submission round and beyond, TACL requires A4
  format.  This is a change from the prior paper size.}

  \item Violation: main document text smaller than 11pt, or table or figure
  captions in a font smaller than 10pt. See Table \ref{tab:font-table}.

  \item Violation: fewer than seven pages of content or more than ten pages of
  content, {\em including} any appendices. (Exceptions are made for
  re-submissions where a TACL Action Editor explicitly granted a set number of
  extra pages to address reviewer comments.) See
  Section \ref{sec:length}.
  \item Violation: Author-identifying information in the document content or
  embedded in the file itself.
    \begin{itemize}
      \item Advice: Make sure the submitted PDF does \emph{not} embed within it
      any author info: check the document properties before submitting.
      Useful tools include Adobe Reader and {\tt pdfinfo}.
      \item Advice: Check that no URLs (or corresponding websites) inadvertently
      disclose any author information. If software or data is to be distributed,
      mention so in {\em anonymized} fashion.
      \item Advice: Make sure that author names have been omitted
      from the author block. (It's OK to include some sort of anonymous
      placeholder.)
      \item Advice: Do not include acknowledgments in a submission.
      \item Advice: While citation of one's own relevant prior work is as
      encouraged as the citation of any other relevant prior work,
      self-citations should be made in the third, not first, person.
      No citations should be attributed to ``anonymous'' or the like.
      See Section \ref{sec:self-cite}.
    \end{itemize}
\end{enumerate}
\fi


\section{General instructions}

\Taclpapers that do not comply with this document's instructions
risk
\iftaclpubformat
publication delays until the camera-ready is brought into compliance.
\else
rejection without review.
\fi


\Taclpapers should consist of a Portable Document Format (PDF) file formatted
for  \textbf{A4 paper}.\footnote{Prior to the September 2018 submission round, a
different paper size was used.} All necessary fonts should be
included in the  file.

\iftaclpubformat
Note that you will need to provide both a single-spaced and a double-spaced
version; see \S \ref{ssec:layout}.

If you promised to provide code or data at submission, specific instructions for
how to access such resources must be provided.  (Typically, a URL to a stable,
resource-specific site suffices.)

All URLs should be manually checked to verify that they
lead to a valid webpage, and to the site that was intended.
\fi


\section{\LaTeX\ files}

\LaTeX\ files compliant with these instructions are available at the
Author Guidelines section of the
TACL website, \href{https://www.transacl.org/}
{https://www.transacl.org}.\footnote{Last accessed \dateOfLastUpdate.} Use of the
TACL \LaTeX\ files is highly recommended: \emph{MIT Press requires authors to
supply \LaTeX\ source files as part of the publication process}; and
use of the recommended \LaTeX\ files makes conversion to the
required camera-ready format simple.
\iftaclpubformat
Specifically, the conversion can be accomplished by as little as: (1) add
``acceptedWithA'' in the square brackets in the line invoking the TACL package,
like so:
{\footnotesize {\tt {\textbackslash usepackage}[acceptedWithA]\{\styleFileVersion\}}} (2) add author information;
(3) add acknowledgments.
\fi

\subsection{Workarounds for problems with the hyperref package}

The provided files use the hyperref package by default. The TACL files
employs the hyperref package to make clickable links for URLs and other references,
and to make titles of bibliographic items into clickable links to their DOIs
in the generated pdf.\footnote{Indeed, for some versions of acl\_natbib.sty,
DOIs and URLs are not printed out or included in the bibliography in any form
if the hyperref package is not used.}

However, it is known that citations or URLs that cross pages can trigger the
compilation error ``{\tt {\textbackslash}pdfendlink ended up in different nesting
level than {\textbackslash}pdfstartlink}''.  In such cases, you may temporarily
disable the hyperref package and then compile to locate the offending portion of
the tex file; edit to avoid a pagebreak within a link;\footnote{If the problematic
link is part of a reference in the bibliography and you do not wish to
directly edit the corresponding .bbl file, a heavy-handed approach is to
add the line
{\tt \textbackslash interlinepenalty=10000}
just after the line
{\tt \textbackslash sloppy\textbackslash clubpenalty4000\textbackslash widowpenalty4000} in the
``{\tt \textbackslash def\textbackslash thebibliography}'' portion
of the file \styleFileVersion.sty.  This penalty means that LaTex will not allow
individual bibliography items to cross a page break.
}
 and then re-enable the
hyperref package.

To disable it,
add {\tt nohyperref} in the square brackets to pass that option to the TACL package.
For example, change
\iftaclpubformat
\verb+[acceptedWithA]+ in
{\footnotesize {\tt {\textbackslash usepackage}[acceptedWithA]\{\styleFileVersion\}}}
to
\verb+[acceptedWithA,nohyperref]+.
\else
{\tt {\textbackslash usepackage}[]\{\styleFileVersion\}}
to
{\tt {\textbackslash usepackage}[nohyperref]\{\styleFileVersion\}}.
\fi



\section{Length limits}
\label{sec:length}

\iftaclpubformat
Camera-ready documents may consist of as many pages of content as allowed by
the Action Editor in their final acceptance letter.
\else
Submissions may consist of seven to ten (7-10) A4 format (not letter) pages of
content.
\fi

The page limit \emph{includes} any appendices. However, references
\iftaclpubformat
and acknowledgments
\fi
do not count
toward the page limit.

\iftaclpubformat
\else
Exception: Revisions of (b) or (c) submissions may have been allowed
additional pages of content by the prior Action Editor, as specified in their
decision letter.
\fi

\section{Fonts and text size}

Adobe's {Times Roman} font should be used. In \LaTeX2e{} this is accomplished by
putting \verb+\usepackage{times,latexsym}+ in the preamble.\footnote{Should
Times Roman be unavailable to you, use
{Computer Modern Roman} (\LaTeX2e{}'s default).  Note that the latter is about
10\% less dense than Adobe's Times Roman font.}

Font size requirements are listed in Table \ref{tab:font-table}. In addition to
those requirements, the content of figures, tables, equations, etc. must be
of reasonable size and readability.
\begin{table}[t]
\begin{center}
\begin{tabular}{|l|rl|}
\hline \bf Type of Text & \bf Size & \bf Style \\ \hline
paper title & 15 pt & bold \\
\iftaclpubformat
author names & 12 pt & bold \\
author affiliation & 12 pt & \\
\else
\fi
the word ``Abstract'' as header & 12 pt & bold \\
abstract text & 10 pt & \\
section titles & 12 pt & bold \\
document text & 11 pt  &\\
captions & 10 pt & \\
%bibliography & 10 pt & \\
footnotes & 9 pt & \\
\hline
\end{tabular}
\end{center}
\caption{\label{tab:font-table} Font requirements}
\end{table}




\section{Page Layout}
\label{ssec:layout}


The margin dimensions for a page in A4 format (21 cm $\times$ 29.7 cm) are given
in Table \ref{tab:margin-table}.  Start the content of all pages directly under
the top margin.
\iftaclpubformat
\else
(The confidentiality header (\S\ref{sec:ruler-and-header}) for submissions is an
exception.)
\fi


\begin{table}[ht]
\begin{center}
\begin{tabular}{|l|}  \hline
Left and right margins: 2.5 cm \\
Top margin: 2.5 cm \\
Bottom margin: 2.5 cm \\
Column width: 7.7 cm \\
Column height: 24.7 cm \\
Gap between columns: 0.6 cm \\ \hline
\end{tabular}
\end{center}
\caption{\label{tab:margin-table} Margin requirements}
\end{table}


\Taclpapers must be in two-column format.
Allowed exceptions to the two-column format are the title, which must be
centered at the top of the first page;
\iftaclpubformat
the author block containing author names and affiliations and addresses, which
must be centered on the top of the first page and placed after the
title; The author names and affiliations must be formatted according
to MIT Press's requirements, which are described in Appendix
\ref{sec:authorformatting}. Using the provided LaTeX style file should
satisfy these requirments.

\else
the  confidentiality header (see \S\ref{sec:ruler-and-header}) on submissions;
\fi
and any full-width figures or tables.

Should the pages be numbered?  Yes, for submissions (to facilitate review); but
no, for camera-readies (page numbers will be added at publication time).

\Taclpapers should be single-spaced.
\iftaclpubformat
But, {\em an additional double-spaced version must also be provided, together with the
single-spaced version, for the use of the copy-editors.}  A double-spaced version can
be created by adding the ``copyedit'' option: Change \verb+[acceptedWithA]+ in
{\footnotesize {\tt {\textbackslash usepackage}[acceptedWithA]\{\styleFileVersion\}}}
to \verb+[acceptedWithA,copyedit]+.
\fi

{Indent} by about 0.4cm when starting a new paragraph that is not the first in a
section or subsection.

\subsection{The confidentiality header and line-number ruler}
\label{sec:ruler-and-header}
\iftaclpubformat
Camera-readies should not include the left- and right-margin line-number rulers
or headers from the submission version.
\else
Each page of the submission should have the header ``\confidentialtext''
centered across both columns in the top margin.

Submissions must include line numbers in the left and right
margins, as demonstrated in the TACL submission-formatting
instructions pdf file, because the line numbering allows reviewers to be very
specific in their comments.\footnote{Authors using Word to prepare their
submissions can create the marginal line numbers by inserting text
boxes containing the line numbers.}
Note that the numbers on the ruler need not line up exactly with the text lines
of the paper. (Indeed, the line numbers generated by the recommended \LaTeX\
files typically do not correspond exactly to the text lines.)
\fi

The presence or absence of the ruler or header should not change the appearance
of any other content on the page.



\begin{table*}[t]
\centering
\begin{tabular}{p{7.8cm}@{\hskip .5cm}p{7.8cm}}
\multicolumn{1}{c}{{\bf Incorrect}} & \multicolumn{1}{c}{{\bf Correct}} \\  \hline
``\ex{(Cardie, 1992) employed learning.}'' &
``\ex{Cardie (1992) employed learning.}'' \\
{The problem}:  ``employed learning.'' is not a sentence.  & Create by
\verb+\citet{+\ldots\verb+}+  or \verb+\newcite{+\ldots\verb+}+. \\
\\  \hline
``\ex{The method of (Cardie, 1992) works.}'' &
``\ex{The method of Cardie (1992) works.}''  \\
{The problem}:  ``The method of was used.'' is not a sentence.  & Create as
above.\\ \\\hline
``\ex{Use the method of (Cardie, 1992).}'' &
``\ex{Use the method of Cardie (1992).}''  \\
{The problem}:  ``Use the method of.'' is not a sentence.  & Create as
above.\\ \\\hline
\ex{Related work exists Lee (1997).} & \ex{Related work exists (Lee,
1997).} \\
{The problem}:  ``Related work exists Lee.'' is not a sentence (unless one
is scolding a Lee). & Create by
\verb+\citep{+\ldots\verb+}+  or \verb+\cite{+\ldots\verb+}+. \\
\\  \hline
\end{tabular}
\caption{\label{tab:cite-commands} Examples of incorrect and correct citation
  format.  Also depicted are citation commands supported by the
  tacl2018.sty file, which is based on the natbib package and
  supports all natbib citation commands.
  The tacl2018.sty file also supports commands defined in previous ACL style
  files
  for compatibility.
  }
\end{table*}





\section{The First Page}
\label{ssec:first}

Center the title, which should be placed 2.5cm from the top of the page,
\iftaclpubformat
and author names and affiliations
\fi
across both columns of the first page. Long titles should be typed on two lines
without a blank line intervening.
\iftaclpubformat
After the title, include a blank line before the author block.
Do not use only initials for given names, although middle initials are allowed.
Do not put surnames in all capitals.\footnote{Correct: ``Lillian Lee'';
incorrect: ``Lillian LEE''.} Affiliations should include authors' email
addresses. Do not use footnotes for affiliations.
\else
Do not include the paper ID number assigned during the submission process.
\fi

\iftaclpubformat
\else
Although submissions should not include any author information, maintain space
for names and affiliations/addresses so that they will fit in the final
(camera-ready)
version.
\fi


Start the abstract at the beginning of the first
column, about 8 cm from the top of the page, with the centered header
``Abstract'' as specified in Table \ref{tab:font-table}.
The width of the abstract text
should be narrower than the width of the columns for the text in the body of the
paper by about 0.6cm on each side.

\section{Section headings}

Use numbered section headings (Arabic numerals) in order to facilitate cross
references. Number subsections with the section number and the subsection number
separated by a dot.



\section{Figures and Tables}

Place figures and tables in the paper near where they are first discussed.
Note that MIT Press disallows figures and tables on the first page.

Provide a caption for every illustration. Number each one
sequentially in the form:  ``Figure 1: Caption of the Figure.'' or ``Table 1:
Caption of the Table.''

Authors should ensure that tables and figures do not rely solely on color to
convey critical distinctions and are, in general,  accessible to the
color-blind.



\section{Citations and references}
\label{sec:cite}


\subsection{In-text citations}
\label{sec:in-text-cite}
Use correctly parenthesized author-date citations
(not numbers) in the text. To understand correct parenthesization, obey the
principle that \emph{a sentence containing parenthetical items should remain
grammatical when the parenthesized material is omitted.} Consult Table
\ref{tab:cite-commands} for usage examples.


\iftaclpubformat
\else
\subsection{Self-citations}
\label{sec:self-cite}

Citing one's own relevant prior work should be done,  but use the third
person instead of the first person, to preserve anonymity:
\begin{tabular}{l}
Correct: \ex{Zhang (2000) showed ...} \\
Correct: \ex{It has been shown (Zhang, 2000)...} \\
Incorrect: \ex{We (Zhang, 2000) showed ...} \\
Incorrect: \ex{We (Anonymous, 2000) showed ...}
\end{tabular}
\fi

\subsection{References}
\label{sec:references}
Gather the full set of references together under
the boldface heading ``References''. Arrange the references alphabetically
by first author's last/family name, rather than by order of occurrence in the
text.

References to peer-reviewed publications should be given in addition to or
instead of preprint versions. When giving a reference to a preprint, including
arXiv preprints, include the number.

List all authors of a given reference, even if there are dozens; do not
truncate the author list with an ``et al.''  Use full first/given names for
authors, not initials.  Include periods after middle initials.

Titles should have correct capitalization.  For example, change change
``lstm'' or ``Lstm'' to ``LSTM''.\footnote{If using BibTex, apply curly braces
within the title field to preserve intended capitalization.}   Capitalize the
first letter of the first word after a colon or similar punctuation mark.  For
book titles, capitalize the first letter of all main words.  See the
reference entry for \citet{Jurafsky+Martin:2009a} for an example.


We strongly encourage the following, but do not absolutely mandate them:
\begin{itemize}
\item Include DOIs.\footnote{The supplied \LaTeX\ files will
automatically add hyperlinks to the DOI when BibTeX or
BibLateX are invoked if the hyperref package is used and
the doi field is employed in the corresponding bib entries.
The DOI itself will not be separately printed out in that case.}
\item Include the version number when citing arXiv preprints, even if only one
version exists at the time of writing.
For example,\footnote{Bibtex entries for \citet{DBLP:journals/corr/cs-CL-0108005} and
\citet{DBLP:journals/corr/cs-CL-9905001} corresponding to the depicted output
can be found in the supplied sample file {\tt tacl.bib}.  We also cite
the peer-reviewed versions \cite{GOODMAN2001403,P99-1010}, as required.}
note the ``v1'' in the following.
\begin{quote}
Joshua Goodman.  2001.  A bit of progress in language modeling. {\it CoRR},
cs.CL/0108005v1.
\end{quote}
An alternative format is:
\begin{quote}
Rebecca Hwa. 1999. Supervised grammar induction using training data with limited constituent
information. {cs.CL/9905001}. Version 1.
\end{quote}
\end{itemize}

\section{Appendices} Appendices, if any, directly follow the text and the
references.  Recall from Section \ref{sec:length} that {\em appendices count
towards the page
limit.}


\iftaclpubformat

\section{Including acknowledgments}
Acknowledgments appear immediately before the references.  Do not number this
section.\footnote{In \LaTeX, one can use {\tt {\textbackslash}section*} instead
of {\tt {\textbackslash}section}.} If you found the reviewers' or Action
Editor's comments helpful, consider acknowledging them.
\else
\fi

\section{Contributors to this document}
\label{sec:contributors}

This document was adapted by Lillian Lee and Kristina Toutanova
from the instructions and files for ACL 2018, by Shay Cohen, Kevin Gimpel, and
Wei Lu. 
This document was updated by Cindy Robinson to
include additional information on formatting final versions.
Those files were drawn from earlier *ACL proceedings, including those
for ACL 2017 by Dan Gildea and Min-Yen Kan, NAACL 2017 by Margaret Mitchell,
ACL 2012 by Maggie Li and Michael White, those from ACL 2010 by Jing-Shing
Chang and Philipp Koehn, those for ACL 2008 by Johanna D. Moore, Simone
Teufel, James Allan, and Sadaoki Furui, those for ACL 2005 by Hwee Tou Ng and
Kemal Oflazer, those for ACL 2002 by Eugene Charniak and Dekang Lin, and
earlier ACL and EACL formats,  which were written by several people,
including John Chen, Henry S. Thompson and Donald Walker. Additional elements
were taken from the formatting instructions of the {\em International Joint
Conference on Artificial   Intelligence} and the \emph{Conference on Computer
Vision and Pattern Recognition}.

\iftaclpubformat

\onecolumn

\appendix
\section{Author/Affiliation Options as set forth by MIT Press}
\label{sec:authorformatting}

Option 1. Author’s address is underneath each name, centered.

\begin{quote}\centering
  \begin{tabular}{c}
    \textbf{First Author} \\
    First Affiliation \\
    First Address 1 \\
    First Address 2 \\
    \texttt{first.email@example.com}
  \end{tabular}
  \ 
  \begin{tabular}{c}
    \textbf{Second Author} \\
    Second Affiliation \\
    Second Address 1 \\
    Second Address 2 \\
    \texttt{second.email@example.com}
  \end{tabular}

  \begin{tabular}{c}
    \textbf{Third Author} \\
    Third Affiliation \\
    Third Address 1 \\
    Third Address 2 \\
    \texttt{third.email@example.com}
  \end{tabular}
\end{quote}
  

Option 2. Author’s address is linked with superscript characters to its name,
author names are grouped, centered.

\begin{quote}\centering
    \textbf{First Author$^\diamond$} \quad \textbf{Second Author$^\dagger$} \quad
    \textbf{Third Author$^\ddagger$}
    \\ \ \\
    $^\diamond$First Affiliation \\
    First Address 1 \\
    First Address 2 \\
    \texttt{first.email@example.com}
     \\ \ \\
     $^\dagger$Second Affiliation \\
    Second Address 1 \\
    Second Address 2 \\
    \texttt{second.email@example.com}
     \\ \ \\
    $^\ddagger$Third Affiliation \\
    Third Address 1 \\
    Third Address 2 \\
    \texttt{third.email@example.com}
\end{quote}
  
\fi


==> tacl_submission_0/sections/dataset.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{figs/gallery.pdf} % Placeholder image
  \caption{\textbf{A} Example rollouts from the dataset. Target CADs (top-center) were shown to \textit{Designers}, who created instructions (left columns) that \textit{Makers} followed (right columns). Dyads iteratively refined their CADs across a series of rounds (rows). \textbf{B} Examples of multimodal refinement instructions. Language and drawing mutually constrain and inform the others' semantics. Many instructions don't make sense without the accompanying drawings, and vice-versa.}
  \label{fig:gallery}
\end{figure*}


\section{The \mrcad{} Dataset}
\label{sec:dataset}

\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{figs/communication_stats.pdf}
  \vspace{-2em}
  \caption{\textbf{A} Designers' instructions to \textit{generate} CADs (round 1) involved lots of drawing and little text, whereas instructions to \textit{refine} CADs (rounds 2+) used a balance of modalities. \textbf{B} The proportions of the types of root words in the dependency parse tree of instruction text. More verbs are used over rounds, and these verbs become more imperative. \textbf{C} Samples of 20 generation drawings and 20 refinement drawings highlights the rich detail in generation instructions, and more targeted modifications in refinement.}
  \label{fig:communication_stats}
  \vspace{-1em}
\end{figure*}

We present the main statistics of our dataset, and a set of basic analyses that reveal the striking effects of multi-modality and refinement on communication. We also include a gallery of multi-modal refinement rounds, highlighting the intriguing yet unexplored aspects of the dataset for future research.

\subsection{Dataset statistics}

% Only CADs that meet our fixed accuracy threshold
The full \mrcad{} dataset contains $3166$ unique CADs recreated by $1092$ dyads.
This resulted in a total of 6082 rollouts (for a sample, see Fig. \ref{fig:gallery} A) with a total of $15163$ rounds of instructions and corresponding executions.
On average, each rollout has $2.49$ rounds, and there are a total of $6078$ generation rounds (round 1) and $9085$ refinement rounds (rounds 2+).
To achieve coverage over diverse CADs while also capturing variance in human communication \cite{ji2022abstract}, our dataset contains three distinct subsets: a \textbf{coverage set}, containing $2249$ unique CADs each successfully reconstructed by $1-2$ dyads; a \textbf{dense set}, containing 698 unique CADs each successfully reconstructed by at $3-6$ dyads; and a \textbf{very-dense set}, containing $27$ unique CADs successfully reconstructed by at least $30$ dyads (Fig. \ref{fig:splits}).
In the following analyses we combine data from the coverage and dense sets, and leave the very-dense set for future work.
% proportion of 1st rounds and refinement rounds?

% avg. maker time
% avg. speaker time

% What proportion met our fixed threshold?
% What proportion met our dynamic threshold?


% the statistics reported in this section are calculated on only these trials.
% XXX trials (XX\%) met our fixed threshold for inclusion in the evaluation set. % report later?

\subsection{Analyzing instructions in \mrcad{}}

\paragraph{Refinements increased accuracy of CADs}
% Our primary measure of reconstruction accuracy was a novel Chamfer distance (see [Supplemental] for full details).
% Inclusion in our dataset required that the accuracy of a reconstructed CAD meet our dynamic submission threshold in a certain round. 
% CADs that required more rounds to meet the threshold were typically less accurate overall, meaning that a simple plot of distance against rounds appears, misleadingly, to have a trend towards worse accuracy across rounds.
% Dividing reconstructions by the number of turns taken to submit reveals a pattern of refinement across rounds (Fig. \ref{fig:splits} B).
A possible concern with implementing a dynamic submission threshold is that dyads may have been able to submit CADs without actually refining their designs, however, we found that, after the initial round, distance to the target continued to decrease ($b=-0.0512$, $t=-16.5$, $p=<0.001$) (Fig. \ref{fig:evals}).
These improvements got smaller as rounds progressed ($b=0.0094$, $t=8.84$, $p=<0.001$). 
Together with the decreasing amount of drawing used across rounds, this suggests that refinements became more fine-grained in later rounds.

\paragraph{Modality use differs in generation and refinement}
Across the 4946 rollouts analyzed, 4125 (83.4\%) contained both text and drawing.
Rollouts containing only drawings made up 14.5\%, and just 2.1\% contained only text, confirming that humans most frequently choose to solve this task using a combination of modalities.
Despite this, many rounds contained only a single modality-- 30.2\% drawing rounds and 16.3\% text rounds.
The distribution of text, drawing, and multimodal instruction was strikingly different in initial generation rounds and subsequent refinement rounds ($\chi^2(2) = 1095, \; p = 0$); almost all generation instructions involved drawings (96.6\%), whereas refinement rounds had a roughly equal split of unimodal text and drawing instructions (Fig. \ref{fig:communication_stats}A).


\paragraph{Refinement drawings are more sparse than generation drawings}
\designer{}s' drawings also changed from generation to refinement rounds.
Most strikingly, \textit{Designers} drew \textit{less} in refinement rounds, as measured by the number of strokes ($b=-5.64$, $t=-72.8$, $p=<0.001$) and amount of digital ``ink'' ($b=20.9$, $t=2.23$, $p=0.026$) used (Fig. \ref{fig:communication_stats}\} B). % in supplemental we should talk about stats used here
Rendering these images also suggest that the \textit{content} of \textit{Designers}' drawings also changed, from mostly complete renderings of target CADs to smaller modifications of sub-parts of the current CAD.
% are these are fundamentally different tasks? In generation you have nothing to work with, in refinement your goal is modification.


\paragraph{Refinement text expresses actions and directives} The text of instructions contained an average of $50.2$ characters, or $9.66$ words. To analyze the difference between the text of generation and refinement instructions, we study the root word of the dependency parse tree. We use the English pipeline of the Stanza NLP package \cite{qi2020stanza} to parse the sentences and extract the root words. We tag the root word based on whether it is a verb, and if so whether the mood of the verb is indicative, imperative, or otherwise. We see in Fig.~\ref{fig:communication_stats}B that generation instructions don't have a verb at the head a majority of the time, while refinement instructions do. The proportion of imperatives -- verbs typically used to express directives issued to a listener -- also increases over the course of refinement turns highlighting how refinement instructions have qualitatively different language from generation.

\paragraph{Multimodal refinement messages}
There are a total of 3723 multimodal refinement messages.
Of these, many contained drawings and text that worked together to convey meaning, such that either modality alone would not be sufficient to convey the same intent (Fig. \ref{fig:gallery}B).
This dataset, along with the \textit{very-dense} subset, provide a resource for future work to investigate how language and drawing are used \textit{together} to communicate precisely.



% XXX trials (XX\%) passed the dynamic threshold and earned a bonus.
% Implementing a dynamic threshold allowed us to collect rounds of modification instructions even when initial CAD reconstructions had high accuracy (Fig. \textbf{supplemental accuracy threshold image?}).



==> tacl_submission_0/sections/discussion.tex <==
\section{Discussion}

We present \mrcad{}, a large-scale dataset of multimodal instructions for generating and refining CADs, and corresponding executions in a CAD environment.
Analysis of these data revealed a difference between instructions to \textit{generate} and instructions to \textit{refine}, CADs, notably a trend towards the complementary use of drawing and text when refining designs.
This distinction is mirrored by a performance gap in model instruction-following for generation and refinement. 

We posit that this is partly due to the lack of multimodal refinement data on the internet, from which these models are trained.
While the internet is a rich source of textual and image data, drawing data is much sparser -- particularly the ephemeral drawings that accompany language.
Furthermore, people typically upload only finished artifacts to the internet, often with accompanying contextual text data, making these datasets well-suited for generation tasks.
On the other hand, the process of editing artifacts based on further instructions is rarely uploaded, which is why these models struggle with interactive refinements.
As a multimodal refinement dataset, \mrcad{} serves as a valuable resource for investigating these phenomena.

% Analyzing these data revealed that drawings were sufficient to convey target CADs, however we consistently observed that participants still choose to use language alongside drawings.
% In the drawing-only condition, \designer{} had few ways of communicating that their drawings suggested the modification of existing elements rather than the addition of new elements.
% This frequently led to the strategy of redrawing the entire target CAD.
% Together, these results suggest that having access to language allowed \textit{Designers} to disambiguate their drawings, making their communication more efficient.
% Even short utterances can hugely constrain the meaning of drawings-- ``delete this'', ``move to here'', ``6 circles along this line''.
% They also highlight the capacity of drawing to act, not only as a depictive medium, but as a rich and versatile tool for \textit{communication} \cite{goodman1976languages, huey2021semantic, fan2023drawing}.

% While humans have generated a large amount of textual data online, drawing data is far more sparse, particularly the kinds of ephemeral drawings that accompany language, which are more akin to gesture than to the myriad photos that are available as training data.



==> tacl_submission_0/sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
% \begin{table*}[]
%     \centering
%     \small
%     \begin{tabular}{lrrrrrrrrrr}
%     \toprule
%     &  & \multicolumn{9}{c}{\textbf{Vision-language models}} \\
%     \cmidrule(lr){3-11}
%     & \textbf{Human} & \textbf{GPT-4o} & $-\text{drawing}$ & $-\text{text}$ & \textbf{Claude} & \textbf{GPT-4o-mini} & \textbf{Qwen} & \textbf{Qwen FT} & & \\
%     \midrule
%     generation & 0.85 & 0.55 & & & 0.50 & 0.31 & 0.12 & 0.43 & & \\
%     refinement & 0.12 & -0.12 & & & -0.05 & -0.13 & -0.05 & -0.02 & & \\
%     \bottomrule
%     \end{tabular}
%     \caption{Proportional improvement results for vision-language chat models. Claude results are from Claude-3.7-Sonnet, and Qwen results are from Qwen2.5-VL-7B-Instruct. Qwen-7B FT is a Qwen2.5-VL-7B-Instruct model fine-tuned on mrCAD data.}
%     \label{tab:api_results}
% \end{table*}

We evaluate both API access models and open-weights models (which we finetune) on the \mrcad{} dataset. 
We are interested in the following.
\begin{enumerate}[label=\textbf{RQ\arabic*},labelindent=0pt,leftmargin=*,itemsep=0pt,parsep=0pt]
    \item What is the difference in performance between people and models in following the instructions?
    \item What is the effect of generation vs refinement in model performance ?
    \item What is the effect of multi-modal vs single-modal in model performance?
\end{enumerate}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\textwidth]{figs/evals.pdf} % Placeholder image
  \caption{\textbf{A} Comparison of human and model movement towards target following instructions, normalized by distance at start of round. Only humans make reliably positive changes in responses to refinement instructions. Models made positive steps in generation but largely destructive changes when refining. \textbf{B} Comparison of human and model responses.}
  \label{fig:evals}
\end{figure*}

\subsection{Benchmark}
We select CADs from the \textbf{dense set} that have 3 or more successful ($\Delta(D_n, D^*) < 0.2$) rollouts.
This results in $682$ unique CADs with $2324$ rollouts, and a total of $5751$ rounds of instruction-execution pairs.
Then, for these selected rounds, we can evaluate VLM agents by having them assume the role of a human maker $P_\text{maker}$.

\paragraph{Metric}
We evaluate the instruction-following abilities by proportional improvements \textbf{PI}: how much the distance to target $D^*$ shrinks as a consequence of an agent's actions.
\begin{align*}
    \text{PI}(A, R_{:i}, D^*) &= \frac{\Delta(D_i, D^*) - \Delta(A(D_i), D^*)}{\Delta(D_i, D^*)}
\end{align*}
This metric is proportional w.r.t. the amount of remaining distance to target at every round.
This accounts for the fact that distances to the target decrease significantly as rounds progress, making late-stage refinements less noticeable without this normalization.

\subsection{Evaluating vision-language models}

We build a gym framework for standardized evaluations across models. The gym framework allows for instantiating agents that interface with a standardized representation of CADs, and allows for handing the mrCAD dataset, evaluating models, and simulating interactions between designer and maker agents.

We use the gym framework to evaluate multiple vision-language chat models -- both API access and open weights models -- on the mrCAD benchmark, by having these models assume the role of a human maker.
% \begin{small}
    \begin{align*}
        P_\text{model-maker}(A ~|~ m, D_i, R_{1:i-1})
    \end{align*}
% \end{small}

\paragraph{API access models} 
Since we present the rendered interaction history and drawing instructions to the model, we require models that are accept interleaved image-text inputs. We choose the following models off-the-shelf based on this criterion: GPT-4o \cite{openai2024gpt4ocard}, GPT-4o-mini \cite{openai2025gpt4omini}, Claude-3.7-Sonnet \cite{anthropic2025claude37}, and Qwen2.5-VL-7B-Instruct \cite{bai2025qwen25vltechnicalreport}.
To generate editing actions, we prompt the models to generate editing actions as tool calls. 

\paragraph{Finetuned Model}
We also fine-tune a Qwen2.5-VL-7B-Instruct model in the same setting to generate editing actions. We use the 2684 rollouts from the coverage set as a training set. We also include rollouts that don't pass the evaluation threshold. We create a small held-out validation set by choosing 303 successful rollouts from the dense set for 187 CADs that have fewer than 3 successful rollouts for model selection. We train LoRA \cite{hu2022lora} adapters for both vision and language modules of the network.

\begin{table}[]
    \centering
    \begin{tabular}{lrr}
        \toprule
         & \textbf{generation} & \textbf{refinement} \\
        \midrule
        Human & 0.85 & 0.12 \\
        \midrule
        GPT-4o & 0.55 & -0.12 \\
        $-\text{drawing}$ & 0.51 & -0.16 \\
        $-\text{text}$ & 0.54 & -0.12 \\
        \midrule
        Qwen-7B FT & 0.43 & -0.02 \\
        $-\text{drawing}$ & 0.36 & -0.03 \\
        $-\text{text}$ & 0.41 & -0.04 \\
        \midrule
        GPT-4o-mini & 0.31 & -0.13 \\
        Claude-3.7 & 0.50 & -0.05 \\
        Qwen-7B & 0.12  & -0.05 \\
        \bottomrule
        \end{tabular}
        \caption{Proportional improvement results for vision-language chat models, including results on ablated instructions. Claude results are from Claude-3.7-Sonnet, and Qwen results are from Qwen2.5-VL-7B-Instruct. Qwen-7B FT is a Qwen2.5-VL-7B-Instruct model fine-tuned on mrCAD data. 
        % For GPT-4o, we only evaluate with the ablated instructions from the evaluation set, while for Qwen-7B FT we fine-tune the model on the training set with the corresponding modality ablated.
        All models perform worse than humans in following instructions, especially instructions of refinements, where the models' outputs actually make the design worser.
        }
    \label{tab:ft_results}
\end{table}

\paragraph{Ablation on modality}
We ablate one modality (if present) from all the instructions and evaluate them to create $-\text{drawing}$ and $-\text{text}$ evaluation sets. We also perform these ablations on the training data and fine-tune separate Qwen2.5-VL-7B-Instruct models to obtain $\text{Qwen-7B FT}_{-\text{drawing}}$ and $\text{Qwen-7B FT}_{-\text{text}}$ models to 
evaluate on the $-\text{drawing}$ and $-\text{text}$ evaluation sets respectively. We use the same LoRA fine-tuning setup for these experiments.

\subsection{Performance of vision-language models}
For the results, we group rounds as either generation (round 1) and refinement (round 2+). 
Note that this grouping is imprecise and can be improved in future works, as participants do instruct each other to generate in later rounds.

\textbf{RQ1, RQ2} We found (Table~\ref{tab:ft_results}) that models are generally able to decrease the distance to the target during \textit{generation}, with more capable models (GPT-4o, Claude-3.7-Sonnet) and fine-tuned models doing better. However, we find that models perform quite poorly in \textit{refinement} turns. We see that models often make changes that actually \emph{increase} the distance to the target -- in opposition to the intention of the designer's instruction. 
We also see that while an approach like supervised fine-tuning leads to significant improvements in generation turns, the gains don't transfer to refinement turns. This suggests that more sophisticated training approaches might be needed to tackle refinement.

\textbf{RQ3} We also see that models are sensitive to both instruction modalities (Table~\ref{tab:ft_results}), with performance descreasing when a multimodal instruction is ablated to have only a single modality. This effect is more pronounced in generation rounds.

% We found that models were able to decrease distance to the target in generation rounds (Fig.~\ref{fig:evals}A).
% Furthermore, these changes seemed somewhat sensible (Fig.~\ref{fig:evals}B), \textbf{explain the good things it did}.
% However, models were not able follow refinement instructions in a way that decreased distance to the target.
% \textbf{explain any good refinements it did do, and why it appears to be failing}.

% We should really have a baseline to make claims that generation rounds are better than nothing
% It's impossible to make negative changes in round 1

% In discussion: it should not be surprising that models cannot do this, given that data of this type is lacking. \ref{tab:ft_results}





==> tacl_submission_0/sections/experiments.tex <==
\section{Effects of Multimodality and Refinement on Communication}
\label{sec:effects-of-multimodality}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{figs/experiments.pdf} % Placeholder image
  \vspace{-2em}
  \caption{\textbf{A}: reconstruction accuracy for the 4 communication conditions --- multimodal+refinement, text only + refinement, drawing only + refinement, and multimodal + generation only. Using text only was less effective. Having no refinement was less effective.
  With refinement, drawing only and multimodal are comparable in performance.
  \textbf{B}: usage of text across rounds --- in the multimodal condition, participants used more texts in the later refinement rounds, suggesting a usage of text in conjunction with drawings to communicate refinements.
  \textbf{C}: usage of drawing across rounds --- in the multi-modal condition, participants used more drawing in the generation round, and less in the refinement rounds.
  % Using only text was less effective at communicating refinement than using drawing or drawing plus text. When only one communication modality was available, it was used to a similar extent across generation and refinement rounds. When two modalities were available, participants appeared to prioritize drawing in early rounds, and increase their use of text in later rounds.
  }
  \label{fig:experiments}
\end{figure}

How do multimodality and refinement each support efficient communication?
Prior to collecting our large-scale dataset, we conducted a set of human ablation studies to answer these questions, manipulating the availability of (1) communication modalities, and (2) refinement rounds.
% By intervening on the maximum number of game rounds
% How is successful communication of a design goal impacted by the availability of a) iterative refinement, and b) multimodal communication? 

% The \designer{} was shown CADs, one by one, and asked to send instructions to the \maker{}.
% The \maker{}, who could not see the target design, followed instructions by placing graphical elements-- 3-point arcs, lines, and circles-- in a CAD interface, and sent these back the \designer{}.
% In two further rounds, the \designer{} sent additional \textit{refinement instructions}, explaining how to edit the current CAD to more closely match the target.

\subsection{Experimental methods}
Crowd source participants were paired and randomly assigned the role of \designer{} or \maker{}. 
We sampled 100 CADs from the Sketchgraph dataset \cite{seff2020sketchgraphs}, and presented these CADs across the set of dyads in each of four conditions:

\paragraph{\textit{multimodal + refinement}}
\designer{}'s messages could include text (up to 200 characters) and/or drawing instruction (unlimited). There are 3 rounds total, each round with 30 seconds for the \designer{} to construct a message, and 120 seconds for the \maker{} to manipulate the current CAD in a CAD interface.

\paragraph{\textit{text only + refinement}}
Where the message could only contain text but not drawing.

\paragraph{\textit{drawing only + refinement}}
Where the message could only contain drawing but not text.

\paragraph{\textit{multimodal + generation only}}
Here, rather than having 3 rounds of communication, they are aggregated into a single big round, with 90 seconds for the \designer{} and 360 seconds for the \maker{}.

% To assess the value of \textit{multimodal} instructions, we included a full \textit{multimodal} refinement condition, in which \designer{}'s instructions could include text (up to 200 characters) and/or drawing instruction (unlimited), as well as two ablated uni-modal refinement conditions- \textit{text-only} and \textit{drawing-only}.
% In the three refinement conditions, \textit{Designers} could send instructions across 3 rounds of 30 seconds each, and \textit{Makers} had between 30 and 120 seconds to create and edit graphics in response.
% To assess the value of refinement within the context of multimodal communication, we also included a \textit{non-refinement} condition, in which \designer{}s had a single round of 90 seconds to send instructions, and \textit{Makers} had up to 360 seconds to respond.

\subsection{Results}

\paragraph{Refinement improves reconstruction}
Participants in all \textbf{refinement} conditions were able to improve their reconstructions over all three rounds ($b=-0.0335$, $t=-6.91$, $p=<0.001$) (Fig. \ref{fig:experiments}A).
While participants in the multimodal refinement condition on round one generated less accurate CADs than the \textbf{generation only} condition ($t=1.47$, $p = 0.145$), by round three their designs were reliably more accurate ($t=-2.15$, $p = 0.0340$), despite having the same total time available.
This highlights the value of iterative refinement for creating accurate designs.

\paragraph{Drawings improves reconstruction}
Participants who could only use text achieved considerably less accurate reconstructions than those in the drawing-only and multimodal conditions ($b=0.127$, $t=6.54$, $p=<0.001$).
While text is a relatively poor communicative medium on its own, participants in the multimodal condition still opted to use text in conjunction with drawings, and increased their use of text in later rounds (Fig. \ref{fig:experiments}B), suggesting that language is useful for \textit{refining} CADs.
The amount of drawing remained consistent in the drawing-only condition, but dropped precipitously after round 1 in the multimodal condition (Fig. \ref{fig:experiments}C).
Overall, when given a choice of multi-modality, human participants favored more drawing for the generation round, and more texts in the refinement rounds.
% This appeared to mark a qualitative transition from instructions asking for the \textit{generation} of a CAD, to instructions requesting \textit{refinement}.

\paragraph{Interim discussion}
Why do participants choose to use multi-modal instructions when given a choice? 
Manually inspecting the data revealed that drawings are primarily used in two ways: Those used for creating a shape, and those used for editing a shape.
In the multimodal condition, the \designer{} can disambiguate these with texts such as ``make this shape'' or ``move the shape as shown''.
However, in the drawing only condition, the \designer{} frequently resorted to redrawing the entire target CAD from scratch --- a valid yet inefficient strategy.
Data collected from this experiment hint towards a complex interplay between linguistic and graphic communication that differs in generation and refinement settings.
The mrCAD dataset, discussed next, aims to provide a large scale dataset of \textit{multimodal generation and refinement instructions} to study these phenomena.

% % Training models that understand the rich interplay between communicative modalities will likely require more than combining separately trained language and image models.
% Evaluating whether models can understand these forms of communication, as well training them to overcome and shortcomings, requires a kind of data that is lacking in the public domain.
% While humans have generated a large amount of textual data online, drawing data is far more sparse, particularly the kinds of ephemeral drawings that accompany language, which are more akin to gesture than to the myriad photos that are available as training data.
% Likewise, while labels often exist for complete CADs and other assets, or can be generated fairly easly using VLMs, language describing the process of \textit{modification} is harder to find.
% % gap: datasets that you can train on and evaluate with
% The mrCAD dataset aims to fill these gaps by providing a dataset of \textit{modifications} with accompanying \textit{multimodal instructions}.
% Such a dataset could be used to train and evaluate multimodal instruction following.


==> tacl_submission_0/sections/intro.tex <==
\section{Introduction}

Recent advances in generative AI have enabled collaborative design via a natural language interface, with applications such as generating images and code.
However, while these models demonstrate impressive results in generating high-quality content, they struggle to \textit{modify} what they have generated based on further user refinement instructions. 
The challenge of getting models to perform interactive edits is well-documented in tasks such as image editing \cite{fu2024guiding} and code generation \cite{cassano2023can}.
This often results in frustration with AI-generated content that is ``nearly there'' but difficult to refine to exactly how the user wanted it.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{figs/opening_fig.pdf} % Placeholder image
  \caption{We present a dataset of multimodal instructions for creating and modifying computer aided designs, along accompanying executions of these instructions in a 2D CAD environment. Participants worked together to recreate a target CAD over multiple rounds. Crucially, the target design is known only to the designer, who must instruct the maker on what to create. The maker, in turn, must edit the CAD model based on these instructions.}
  \vspace{-1em}
  \label{fig:opening}
\end{figure}

On the other hand, humans regularly instruct each other to perform refinements.
Works such as \citet{dingemanse2024interactive} have argued that since human communication is infinitely expressive, repair is a core mechanism for ensuring robust communication.
Further, human-given refinements are often multimodal \cite{lawson2006designers, williams2002designers} where different modalities interact to make the instruction precise.
% Despite the importance and richness of refinements, prior work on the topic [cites] has been largely observational, with only hundreds of instances, making it difficult to conduct a systematic analysis of the nature of refinements, let alone explore ML approaches such as supervised fine-tuning.

We present \mrcad{}, a resource for studying and benchmarking multi-modal refinement in a computer-aided design (CAD) setting. 
An example data-point is shown in Figure \ref{fig:opening}. 
One player, the \emph{Designer}, has a target design which they demonstrate via a combination of text and drawing instructions. The other player, the \emph{Maker}, uses a programmatic CAD language to carry out the Designer's instructions and attempt to recreate the target. In subsequent rounds, the Designer and Maker iteratively \emph{refine} the design to get closer to the target.

Our task setup produces both (1) natural interaction between modalities: e.g.\ in Figure 1, the text specifies `lines have to be straight' and the drawing specifies \emph{which} lines need to be straight and (2) contextual dependence, where refinement instructions need to be interpreted in the context of what has been constructed so far.
People naturally use both types of context when generating and interpreting instructions (Sec.\ \ref{sec:effects-of-multimodality}); but we find that models struggle particularly with refinement (Sec.\ \ref{sec:evaluation}).
% \dfcomment{can we talk through this a bit: the Designer has a target intent, which they demonstrate via drawing and a text instruction. The Maker uses a programmatic CAD language...}
% We believe \mrcad{} can serve as a valuable resource both for benchmarking VLM models, and for understanding the nature of multi-modal refinements.

\paragraph{Benchmarking} As a grounded instruction-following benchmark, \mrcad{} benefits from the programmatic representation of CAD.
CAD reconstruction accuracy can be programmatically defined, in contrast to image creation tasks, which rely on learned metrics such as CLIP~\cite{radford2021learning}.
Additionally, CAD programs can be easily manipulated using a sequence of simple clicks and drags, making it easy to evaluate both tool-using agents and human participants in an evaluation environment.

\paragraph{Understanding} As a resource for understanding the nature of multimodal refinement in human-human collaboration, 
\mrcad{} is large scale, containing 6,082 human-to-human plays of the game, with a total of 15,163 instruction-execution rounds. %, for a total of yyyy man-hours of annotation efforts.
A large number of CADs in our dataset are recreated \emph{multiple} times by different dyads, ranging from 2 to 30 games per CAD design. %3 recreations all the way to 30.
% \dfcomment{it may be hard for people to understand `recreation' unless we mention that this is a reference game with a target image in mind -- but see my comment above about talking through Fig 1. }
This way, we can understand the variation in refinement strategies across people. 
The CAD designs in \mrcad{} are naturalistic, sourced from the SketchGraphs dataset \cite{seff2020sketchgraphs}, consisting of 2D CAD created by designers.
A notable feature of CAD is that while it only contains simple curves of lines, circles, and arcs, put together these simple curves form rich semantic objects and sub-parts (like the ``flower'' and ``petals'' in Figure \ref{fig:opening}), which must be parsed contextually \cite{ji2022abstract}.
This is in contrast to other scene creation datasets such as \citet{zitnick2013bringing}, where each object in the scene has a canonical, pre-defined name (e.g. a ``boy'' and a ``ball'').
The instructions we collect in \mrcad{} consist of freeform drawings and text, highlighting how humans leverage multimodality and refinement in an open-ended manner.

Our work makes the following contributions:
\begin{itemize}[]
    \item A novel task of multi-modal refinement of CAD designs.
    \item A detailed procedure for collecting a dataset of multi-modal refinement communications using crowd-sourcing.
    \item The dataset and benchmark, consisting of 15,163 instructions and executions, wrapped in an accessible gym environment.
    \item Analyses of human-human communication that reveal differences in the multimodal languages of generation and refinement.
    \item Evaluation of existing VLM models, revealing a severe gap in their refinement ability, particularly compared to their generation ability.
\end{itemize}



==> tacl_submission_0/sections/procedure.tex <==
\section{Data Collection Procedure}

% Top level problem
% Now we have validated a method for collecting multimodal refinement instructions, 
How can we scale-up the previous study to maximize the number of high-quality multimodal refinement instructions?
Ensuring quality in a dataset of this size involved multiple competing goals: collecting large volumes of high-quality data, minimizing costs, and fairly compensating crowd workers with varying degrees of effort and skill.

% Our goal for this dataset was to maximize the number of high-quality instruction and editing sequences, while exposing the phenomena of multimodal communication and refinement.
% To collect larger volumes of multimodal instructions and corresponding edits, we converted the mrCAD task into a two-player online game.

\subsection{mrCAD annotation task}
We recruited fluent English speakers from the USA and UK on Prolific.
Participants were paired, randomly assigned the role of \designer{} or \maker{}, and worked together over a series of rounds to recreate target CADs.
Rather than fixing a number of rounds and the amount of time per round, we instead limited the maximum round number to 10, and time to 9 minutes.
Within these limits, participants can choose how many rounds they will take, and to allocate different amount of times for each round.
We also lifted the limit on the amount of text characters the participants can send in a message.
% For distance metric, we used chamfer distance, as some of the CADs may have overlapping or imperceptible (e.g. a line vs a very shallow arc) geometries, making programmatic distance inaccurate.

% The \designer{} was shown CADs, one by one, and asked to send a text and/or drawing instruction to the \maker{}.
% The \maker{}, who could not see the target design, then followed these instructions by placing graphical elements-- 3-point arcs, lines, and circles-- in a CAD interface, and sent these back the \designer{}.
% If the \textit{Makers}' CAD was sufficiently accurate (see next section), the \designer{} could submit this design to each earn a \$1 bonus and advance to the next CAD.
% Otherwise, the \designer{} had to send additional \textit{refinement instructions}, explaining how to edit the current CAD to more closely match the target.
% These refinement instructions could also contain text and/or drawings, this time directly on top of the Maker's design.

\subsection{Sampling CAD tasks}
% Some real-language about why sketchgraph
% To collect a diverse set of tasks, we sampled 6k distinct CADs from the Sketchgraph dataset, with $5$-$25$ graphical elements each --- Our pilot suggested CADs with this number of elements would be sufficiently complex to require multi-turn interactions to communicate effectively, while not being too complex for the average crowd worker.
% To ensure these CADs are absolutely distinct, we first hash the CADs to distinct buckets grouped by curve types, and then choose one from each bucket.
% For example, there is only one CAD in our set of 6k with 4 lines, 2 arcs, and 2 circles.
We sample tasks from the SketchGraphs dataset \cite{seff2020sketchgraphs}. 
%The dataset contains around 15 million designs created by people and shared online. We identify a subset of the SketchGraphs data that has designs that exhibits variety of shapes, and has a range of difficulty that is suitable for participants in our task to complete within the constraints of time and the CAD construction interface. 
We first normalize all designs to a 20 $\times$ 20 grid to identify duplicates. We then rescale the designs by a random scaling factor to ensure a variety of design sizes, while ensuring a minimum gap between pairs of elements such as control points, parallel lines, and concentric arcs or circles to ensure that they were far enough apart to be reproducible in the CAD construction interface. 
We then grouped designs into buckets based on a `signature' determined by the count of various types of curves in the design (horizontal lines, vertical lines, skewed lines, arcs, and circles). 
By selecting one design per bucket, we: (1) eliminated most near-duplicates (2) select a more diverse set of designs.
% This allowed eliminating most near-duplicates, and allows allowed us to select a more diverse subset of tasks by sampling one or a few tasks from each group.
Participants were given 12 tasks randomly sampled from the task pool and shown in order of increasing difficulty (increasing number of curves in the design). 

\subsection{Prioritizing motivated annotators}
The \mrcad{} task is challenging.
Successful performance requires a person to (1) learn to operate a new CAD interface and (2) be adept at communicating CAD modifications, all within the span of one online session.
Furthermore, in a two player game, \emph{both} players must be motivated and capable for a successful reconstruction.
How can we prioritize capable dyads to provide high-quality annotations, while fairly compensating capable individuals with an unmotivated partner? 
We devised an incentive scheme as follows.
% that compensates capable individuals with a base pay irrespective of their partner's performance, and bonus payment for the dyad dependent on the number of successful recreations.

\paragraph{Prioritizing capable individuals}
Before participants started performing CAD tasks, they had to pass through three checks: a comprehension quiz, a solo CAD reconstruction task, and a paired practice trial.
In the solo CAD reconstruction task, each participant has to recreate a simple CAD consisting of a line, circle, and arc, to our fixed threshold level of accuracy.
All participants who passed the solo reconstruction task are deemed capable and motivated, and received a base pay of (\$8.70).

\paragraph{Prioritizing capable dyads}
Once paired, dyads had to successfully recreate one practice trial (a simple smiley face) in order to attempt other CADs.
We awarded a \$1 bonus per person for every recreation that met the accuracy threshold.
If a dyad fails to meet the threshold in 9 minutes, they lose a ``life''.
Dyads were ejected from the study when they lose 3 lives, limiting the number of CADs that unmotivated dyads could attempt.
This scheme directs our compensation towards high quality reconstructions from capable dyads.

\subsection{Prioritizing refinement instructions}
% \paragraph{Threshold for submitting CADs}
Our primary goal was to collect a large number of \textit{multimodal refinement instructions} that led to high-quality reconstructions.
A simple way of ensuring high-quality reconstructions it to implement a fixed threshold of accuracy for submitting CADs.
However, this fixed threshold does not take into account that some CAD would be easier to reconstruct while others would be more challenging.
In a pilot study, we found that with a lenient threshold, unmotivated dyads submitted low quality reconstructions \emph{without refinements}, while with a stringent threshold, motivated dyads were not compensated for decent quality reconstructions on more complex CADs.

Therefore, we implemented a \textbf{dynamic submission threshold}, which allowed only highly accurate reconstructions to be submitted in early rounds, but was more permissive in later rounds.
Implementing this change allowed us to collect 1,532 additional refinement rounds, an increase of 10.1\% compared to using a static threshold.
Furthermore, a dynamic threshold kept motivated dyads who had been "stumped" by a difficult CAD in the study longer by not losing a life.
The effect of dynamic threshold can be see in Figure \ref{fig:splits} B.

\subsection{Exclusion criteria}
Rollouts that contained no CAD actions, entirely empty messages, or had missing rounds were excluded from the dataset for analysis.
We also imposed a fixed \textbf{inclusion threshold} (Figure \ref{fig:splits} A) on reconstruction accuracy for analysis.
In the statistics below, we report only data that meets these criteria, however our full dataset release also includes failures and practice trials.


% \subsection{Annotators}


% By implementing early performance filters, bonusing participants for successful reconstructions, limiting the amount of failures, and implementing a dynamic submission threshold, we were able to collect large volumes of multimodal refinement instructions.
% Summarize with "if we didn't do these tricks, it would have cost X. But it cost Y"

\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{figs/dataset_stats.pdf} % Placeholder image
  \caption{
  \textbf{A} The \mrcad{} dataset contains three subsets: the \textbf{coverage set} of 2249 CADs with 1-2 successful rollouts, \textbf{dense set} of 698 CADs with 3+ successful reconstruction, and the \textbf{very-dense set} of 27 CADs with 30+ successful reconstruction.
  \textbf{B} We implemented a dynamic threshold for submitting designs that became more lenient in later rounds. Participants took a variable number of rounds to reach the threshold. Visualizing distance to the target broken down by round submitted reveals a trend of refinement over time.
  Red dashed line indicates the fixed threshold for including in analysis.
  % A. Dyads successfully refined CADs over multiple rounds, and could submit their CAD once they reached the threshold, which became more lenient as rounds went on. Only CADs that meet our fixed threshold are included in the full \mrcad{} dataset. 
  }
  \label{fig:splits}
\end{figure}

==> tacl_submission_0/sections/related.tex <==
\section{Related Work}

\paragraph{Multimodality}
The instructions in \mrcad{} are multi-modal, consisting of both texts and drawings. 
This is in contrast to other works such as \citet{pejsa2016room2room} and \citet{ku-etal-2020-room}, where the context of the agent is multi-modal, yet the instructions themselves only contain language.
% Our dataset contains many examples of drawings and text that mutually support each other. 
Our drawings efficiently convey spatial information and reference, and even short utterances -- ``delete this'', ``move to here'' -- can hugely constrain the meaning of drawings.
Our work highlights the capacity of drawing to act, not only as a depictive medium, but as a versatile tool for \textit{communication} \cite{goodman1976languages, huey2021semantic, fan2023drawing}, and provides a resource for studying this phenomenon in a grounded way \cite{lachmy2022draw}.

\paragraph{Generating Designs} 
Prior work has explored AI agents that assist with computer aided design tasks, including those that leverage various kinds of input modality \cite{sanghi2022clip, chen2024generic}, including drawings \cite{seff2021vitruvion}. 
Beyond CAD, other work has explored how agents can support various kinds of designs given multimodal inputs, including generating HTML and CSS code \cite{si2024design2code} and slide-shows \cite{ge2025autopresent}. 

\paragraph{Refinement}
The interactions between people in \mrcad{} takes multiple turns, as a dyad collaboratively refine a current CAD toward a specific target. 
% This is in contrast to multimodal instruction-following datasets such as \citet{ku-etal-2020-room} containing a single turn of instruction and response. 
\citet{lachmy2022draw} study complex instructions, but these are presented all at once by the speaker and verified with interpretation by another agent. \mrcad{} prioritizes refinement, where people must elaborate on and repair previous instructions, in this regard, our work is similar to \citet{kim-etal-2019-codraw}.


% \citet{si2024design2code} introduce a front-end design benchmark where an agent is tasked with generating HTML and CSS code, given a visual representation of intent -- the screenshot of the desired page. 
% \citet{ge2025autopresent} develop agents that create a slide given a natural language description of the slide. 
% Our work introduces the task of \emph{refining} designs given \emph{multimodal} instructions in the form of drawings and text.
% \cite{zitnick2013bringing} presents a dataset of comic-book like scene, along with a natural language description of parts are parts, cad parts are fluid.



==> tacl_submission_0/sections/task.tex <==
\section{The \mrcad{} Task}

% The \mrcad{} task is a two player, multi-turn communication game where one player, the \designer{}, instructs another, the \textit{Maker}, to take actions in a mutually observable CAD environment, toward a specific goal state.
The \mrcad{} task (Fig. \ref{fig:opening}) is a two player, multi-turn communication game.
Following \citet{mccarthy2024communicating}, a \designer{} issues multimodal instructions to guide a \maker{} to take actions in a mutually observable CAD environment to construct a target CAD.
The target CAD is known only to the \designer{}.

\subsection{\mrcad{} Environment} \label{sec:env}
% The \mrcad{} environment is as follows.

\paragraph{State} The state $D$ is a CAD data structure.
% design consisting of a set of curves, where each curve can be either a line, circle, or an arc.
\begin{lstlisting}
D -> {Curve, ...}
Curve  -> Line | Circle | Arc 
Line   -> l(P,P) // end points
Circle -> c(P,P) // points on diameter
Arc    -> a(P,P,P) // start, mid, end
\end{lstlisting}
Each curve is defined by its \emph{control points} that the \maker{} selects. 
% A line defined by its end points. A circle by two end points on its diameter. An arc is defined by three points -- two end-points and a mid-point that the arc passes through.
A \texttt{render} function allows players to view the state by rendering the design as an image.
% Each design can be rendered $r(D)$ into an image for display to the players. 
% The starting state is the empty design $D_0 = \{\}$.

\paragraph{Action} The \maker{} can alter the CAD by making, removing, and moving curves via translation.
They can also change the shape of a curve by moving its control points. 
If multiple curves share the same control point, moving the point would modify all the curves, and deleting the point would delete all the curves.
\begin{lstlisting}[mathescape=true]
Action -> make_curve Curve 
        | remove_curve Curve 
        | move_curve Curve Vxy
        | move_point P P
        | delete_point P
\end{lstlisting}

% Note that these are the actions we provided to human players of the game through a web interface and is a small but expressive set of actions. Future work could explore more sophisticated, hierarchical, and dynamic action spaces \cite{mccarthy2021learning}.

\paragraph{Transition} A sequence of actions $A = [a_1, a_2, \ldots, a_n]$ can be applied to a design, which results in a new design.
% \begin{small}
\begin{align*}
    D' &= A(D) = [a_1, a_2, \ldots, a_n](D) \\
    &= (a_n \circ \cdots \circ a_1)(D)
\end{align*}
% \end{small}

\paragraph{Distance Metric} 
% \mrcad{} offers 2 kinds of distance metrics, programmatic and geometric. Programmatic distance serves as a proxy for the amount of actions it requires for a user to alter one design to another one. Given two designs, it first performs a pair-wise matching on the curve types of the two designs (line matched to the nearest line, arc matched to the nearest arc, etc). It then aggregates the amount of movements required to move one curve's control points to match the another curve (see Figure \ref{fig:dist_metric} (left)). 
% Geometric distance compliments the programmatic distance, in cases where the curve types of the two designs \emph{do not} exactly match. For instance, a user might use a straight line to represent a shallow arc. \mrcad{} uses chamfer distance to measure geometric similarity. Given two designs, A and B, chamfer distance computes how much every (sampled) point in A has to move until it ends up in B. To ensure symmetry, both distances average from A to B and from B to A. Details of the implementation of these metrics can be found in the Appendix [ref]. 
CADs are programmatic entities that exist in a visual space, where very different elements could be used to create two CADs of similar appearance.
For example, a series of straight lines can be used to represent a curve.
Therefore, we devise a distance metric $\Delta$ based on chamfer distance \cite{butt1998optimum} that respects the vector-like nature of CADs, while accounting for geometric similarity (Fig. \ref{fig:dist_metric}).

% , in cases where the curve types of the two designs \emph{do not} exactly match. For instance, a user might use a straight line to represent a shallow arc. \mrcad{} uses chamfer distance to measure geometric similarity. Given two designs, A and B, chamfer distance computes how much every (sampled) point in A has to move until it ends up in B. To ensure symmetry, both distances average from A to B and from B to A. Details of the implementation of these metrics can be found in the Appendix [ref]. 


\begin{figure}[t]
  \centering
  \includegraphics[width=0.3\textwidth]{figs/chamfer_distance.pdf} % Placeholder image
  \caption{The \textbf{asymmetric chamfer distance} from CAD $D$ to CAD $E$ is calculated by sampling 10 points on every curve of $D$, and calculating (symbolically) the minimum distance from each point to $E$.
  Each distance is then normalized by multiplying $\frac{1}{4}$ of the maximum size of the canvas, making it invariant to the canvas size.
  These distances are summed, making the asymmetrical chamfer distance.
  The symmetric Chamfer distance we use is the average of both directions.
}
\vspace{-1em}
  \label{fig:dist_metric}
\end{figure}
% Programmatic distance (left) and Chamfer distance (right). Programmatic distance measures the amount of actions it requires to edit design to another, while Chamfer distance measures the designs raw geometric similarity. One advantage of chamfer distance is that it can measure similarity between different curve types, such as the distance from a line to an arc.

\paragraph{Instructions}
The \designer{} can instruct the \maker{} using multimodal messages.
\begin{lstlisting}[mathescape=true]
Message -> $\langle$Text, Drawing$\rangle$
Text    -> [char, ...] | empty
Drawing -> [stroke, ...] | empty
\end{lstlisting}
A text is a sequence of characters and a drawing is a sequence of strokes, encoded in SVG format.

\subsection{Playing the Game}
The shared goal of the \designer{} and \maker{} is to collaboratively reconstruct a target design, which is only given to the Designer.

\paragraph{Round and Rollout} A round is a tuple of: a design $D$, the message from the designer $m$, the actions generated from the maker $A$, and the resulting updated design $D' = A(D)$. A rollout is a sequence of rounds.
% \begin{small}
\begin{align*}
r_i &= (D_i, m_i, A_i, D'_i) \\
R &= [r_1, \ldots, r_n]
\end{align*}    
% \end{small}

Each rollout has $D_1 = \{\}$ and $D_i = D'_{i - 1}$.
A game is ``won'' if the final design is within a certain threshold $\theta$ of distance from the target $D^*$.
% \begin{small}
    \begin{align*}
        \Delta(D'_n, D^*) < \theta
    \end{align*}
% \end{small}

\paragraph{\Designer} At round $i$, the designer is given both the target and current designs, rendered as images f $D^*$ and $D_i$, along with the history of the (rendered) interaction of previous rounds $\texttt{render}(R_{1:i-1})$, and generates a message $m$ from 
% \begin{small}
    \begin{align*}
        P_\text{designer}(m &~|~\texttt{render}(D^*), \\
        & \texttt{render}(D_i), \texttt{render}(R_{1:i-1}))
    \end{align*}
% \end{small}

Presenting designer only the rendered CADs encourages them to focus on the geometric properties and communicate the refinements naturalistically, instead of communicating about the underlying CAD program itself.

\paragraph{\maker{}} The maker takes in the message, the current design, the interaction history, and generates a sequence of actions $A$ from
% \begin{small}
    \begin{align*}
        P_\text{maker}(A ~|~ m, D_i, R_{1:i-1})
    \end{align*}
% \end{small}

\paragraph{Play}
Playing the game starts with  a target design $D^*$ and involves a dyad (a designer-maker pair) acting in turns to generate a rollout.
% \begin{small}
    \begin{align*}
        R = \texttt{play}(D^*, P_\text{designer}, P_\text{maker})
    \end{align*}
% \end{small}
